Fast Uplink Grant-Free NOMA with Sinusoidal Spreading Sequences

Uplink (UL) dominated sporadic transmission and stringent latency requirement of massive machine type communication (mMTC) forces researchers to abandon complicated grant-acknowledgment based legacy networks. UL grant-free non-orthogonal multiple access (NOMA) provides an array of features which can be harnessed to efficiently solve the problem of massive random connectivity and latency. Because of the inherent sparsity in user activity pattern in mMTC, the trend of existing literature specifically revolves around compressive sensing based multi user detection (CS-MUD) and Bayesian framework paradigm which employs either random or Zadoff-Chu spreading sequences for non-orthogonal multiple access. In this work, we propose sinusoidal code as candidate spreading sequences. We show that, sinusoidal codes allow some non-iterative algorithms to be employed in context of active user detection, channel estimation and data detection in a UL grant-free mMTC system. This relaxes the requirement of several impractical assumptions considered in the state-of-art algorithms with added advantages of performance guarantees and lower computational cost. Extensive simulation results validate the performance potential of sinusoidal codes in realistic mMTC environments.

==> sections/introduction.tex <==
\subsection{Background and Motivation}
The sky-rocketing growth in the demands of wireless networks is not anymore limited to enhanced throughput and privacy protection. Rather, it is incorporating many verticals to cater a wide range of distinct use cases. As a consequence, along with enhanced mobile broadband (eMBB) and ultra-reliable and low latency communications (URLLC), massive machine-type communication (mMTC) has been included as one of the major service categories of 5G wireless network in the IMT 2020 Vision Framework by International Telecommunication Union (ITU) \cite{metis}. This made mMTC an extended use case of 5G wireless network. Typical example of mMTC is the collection of massive number of nodes such as smart meters in smart grid, IoT (Internet of Things) network or automated factories \cite{mmtc}.

Unlike human-agent based wireless networks, mMTC exhibits several distinct features in operation. These are: uplink (UL) dominated network, sporadic activity of transmitting nodes, transmission of short sized packets and low data rates \cite{mmtc}. Because of these features, direct translation of conventional grant-access based legacy communication systems lose its relevance in mMTC. Significant signaling overhead associated with grant-acknowledgment scheduling procedures impose higher latency which is another obstacle to realize sporadic transmission of short packets. For example, it has been shown in \cite{ulgf} that in 4G LTE, to transmit a small amount of data (e.g. 20 bytes of data using Quadrature Phase Shift Keying (QPSK) occupying 160 Resource Elements (RE)), the UL grant signaling overhead (\textit{i.e.} 72 REs) to the total resources occupied by the UL grant and UL payload (\textit{i.e.} 72 + 160 REs) can be around 30\%. To tackle these hindrances while supporting massive connectivity, UL grant-free non-orthogonal multiple access (NOMA) schemes, which have drawn significant attention of researchers in recent years, offer promising solutions \cite{noma,noma2,mmtc1,ulgf}. Uplink grant-free NOMA allows devices/users to randomly transmit data without any complex handshaking process while supporting massive connectivity by allocating limited resources in a non-orthogonal manner to massive number of users. 

According to empirical findings, the number of simultaneously active users at a given point of time does not exceed 10\% of the potential users in a wireless network, even in its peak operation time \cite{empirical}. Thus there exists an inherent sparsity in the user activation pattern of mMTC networks. This implication of user sparsity in mMTC led researchers to employ Compressive Sensing (CS) based Multi User Detection (CS-MUD) techniques for active user detection (AUD), channel estimation (CE) and data detection (DD). In practical applications, the user activity pattern remain unchanged over several consecutive OFDMA frames (Orthogonal Frequency Division Multiple Access) which is known as frame-wise sparsity in literature. Several recent works exploited this particular notion of frame-sparsity to derive greedy CS-MUD algorithms like Group Orthogonal Matching Pursuit (GOMP), weighted GOMP (WGOMP) and structured iterative support detection (SISD) \cite{sisd}. These algorithms suffer from exponentially increasing computational complexity hence prohibitive in implementation in large networks. However, several proposed CS-MUD algorithms \textit{e.g}: information enhanced adaptive matching pursuit (IE-AMP) \cite{ieamp}, simultaneous OMP with extrinsic information transfer (SOMP-EXT) \cite{sompext} enjoy much reduced complexity. But these algorithms are reliant on several approximations \textit{e.g}: noise statistics, prior knowledge of sparsity level (number of active users) or perfect channel knowledge at base station (BS) which are not straightforward, if not impractical, to obtain in a real mMTC network.

On the other hand, several researchers proposed Bayesian frameworks for user detection and channel estimation \cite{sbl,map,ep} in mMTC. In \cite{ep} authors proposed expectation propagation (EP) based joint user detection and channel estimation where a computationally intractable Bernoulli-Gaussian distribution was approximated to a tractable multivariate Gaussian to find an estimated \textit{posteriori} distribution of sparse channel vector. In \cite{sbl} authors proposed Sparse Bayesian Learning (SBL) based user detection and channel estimation. Although these Bayesian approaches offer promising performance, a major shortcoming of these methods is their dependence on preset empirical priors \textit{e.g}: user activation probability and the availability of precise statistics of noise and channel gain at BS. In all of these works, either random sequences or Zadoff-Chu sequences were used as spreading sequences. Performance gains can be achieved by optimization of spread sequences but that discussion is out of the scope of this paper. 

In this work, we sought the answer to the question: is it possible to harness the performance guarantees of faster yet accurate classical signal processing algorithms in the active user detection and channel estimation problem in UL grant-free NOMA? Furthermore, we found that it is of paramount importance to develop techniques for AUD, CE and DD in mMTC which are not dependent on any empirical prior or noise/channel statistics so as to improve feasibility along with performance gain. 

\subsection{Contribution}
The contributions of this work can be summarized as following:
\begin{itemize}
    \item We show that it is indeed possible to apply parameter estimation algorithms from signal processing paradigm by using sinusoidal sequence as spreading sequence in UL NOMA systems. The resultant system model contains Vandermonde structure which allows us to apply variants of Multiple Signal Classification (MUSIC) \textit{e.g}: root-MUSIC or rotational invariance based search-free ESPRIT. These subspace estimation based techniques do not require prior noise/channel statistics at the BS. For supporting wide range of active users, we propose using weighted information criteria (WIC) which is based on corrected Akaike information criteria (AICc) and Bayesian Information Criteria (BIC) for model order determination. This is equivalent to determining sparsity level in greedy algorithms. In this way, proposed technique escapes both of the most pressing requirements which are commonly assumed to be met in CS-MUD and Bayesian approaches. For further performance improvement, especially in scenarios with higher number of active users, ESPRIT is used to initialize a non-linear least square optimization via Variable Projection (ESP-VPN) algorithm. To authors' knowledge, this particular perspective has not been addressed in literature before. 
    \item We devise conditions of reliable recovery of transmitted data symbol. In short, among estimated active users (UE) we list UEs of which data symbols cannot be recovered reliably. This may aid MAC (Media Access Control) to derive optimal power control strategies for connected devices
    \item We carry out extensive numerical evaluations in realistic non-line of sight (NLOS) scenarios of mMTC demonstrated by 3GPP (release 9) to compare various performance metrics over several network parameters. It is demonstrated that proposed method outperforms state-of-art Bayesian algorithm \cite{ep} in most of the cases while maintaining less computational expenditure
\end{itemize}
The rest of the paper is organized as following: Section \ref{system_model} demonstrates the system model of an UL grant-free mMTC system. In Section \ref{mod_system_model}, we propose sinusoidal code as spreading sequence and transform the system model. Section \ref{esprit} delineates the methods used for model order selection and active user identification followed by Section \ref{ce_dd} where conditions of reliable data recovery is derived along with channel estimation technique. A detailed numerical investigation is carried out at Section \ref{simulations} where performance comparison and complexity analysis are discussed. We conclude and briefly discuss several future research directions in Section \ref{conclusion}. 

\subsection{Notation}
In the sequel, $\mathbb{B},\mathbb{R}$ and $\mathbb{C}$ represent the fields of binary, real and complex numbers, respectively. In addition, $x$, $\zx$, $\bX$ are used to represent a scalar, a vector, and a matrix, $\zx_j$ denotes the $j^{th}$ column of matrix $\bX$, whereas $\bX(m,n)$ is used to denote the element in $m^{th}$ row and $n^{th}$ column. $\vert\vert\cdot\vert\vert_m$ is used as $\ell_m$ norm operator. $\bI_M$ is an $M\times M$ identity matrix. $\mathcal{CN}(\mu,\bA)$ is used to present complex Gaussian distribution with mean $\mu$ and covariance matrix $\bA$. $\mathrm{\Tr}(A)$ is used to denote the trace of matrix $\bA$. $\vert \cdot \vert$ denotes absolute value or cardinality of a set depending on the context. Elementwise Hadamard product operator is denoted using $\odot$. Moreover, $\diag(\bA)$ is used to denote a matrix having diagonal elements identical with $\bA$, whereas the off-diagonal elements are set to zero. Finally, the probability, expectation and variance operator are denoted as $\Pr(\cdot)$ $\E[\cdot]$ and $\Var[\cdot]$ respectively. 

==> sections/new_model.tex <==
\subsection{Sinusoids as Spreading Sequences}
In this work, we propose using sinusoid based sequences as spreading sequences for non-otrhogonal multiple access. As will be shown in later section, this creates the provision of applying fast subspace algorithms. An element of $i^{th}$ sequence where $\{i\}_{i=0}^{N-1}$ can be expressed as following:
\begin{equation}
    \boldsymbol{\phi}_i(k) = \frac{1}{\sqrt{M}} \exp(\frac{\irm2\pi k}{N}i) \ \  \mathrm{where} \ k \in \{0,1, \cdots M-1\}
    \label{sin}
\end{equation}

The normalizing constant $\frac{1}{\sqrt{M}}$ is used to make the sequence having $\ell_2$ norm $\vert\vert\boldsymbol{\phi}_i\vert\vert_2 = \gamma$. 

\subsection{Signal Model using Sinusoid Sequence}
\label{newmodel}
Using sinusoidal sequence mentioned in \eqref{sin}, the received signal at $m^{th}$ subcarrier where $\{m\}_{m=0}^{M-1}$ in $j^{th}$ frame can be written as 
\begin{equation}
    y_{m,j} = \sum_{n=1}^{\vert\mathcal{N}\vert} h_n\beta_{n,j}\exp(\irm\omega_n m) + w_{m,j}
    \label{append}
\end{equation}
where $\omega_n = 2\pi i/N$ where $i$ is the sequence index associated with the UE $n$. To create signal snapshots of length $l$ from received signal in $j^{th}$ frame, we get $\Bs_{m,j} = [y_{m,j} \ y_{m+1,j} \ \cdots \ y_{m+l-1}]^T$. This can be formulated as following
\begin{equation}
    \Bs_{m,j} = \sum_{n=1}^{\vert\mathcal{N}\vert} h_n\beta_{n,j}\exp(\irm\omega_n m)\boldsymbol{\theta}_n
\end{equation}
where $\boldsymbol{\theta}_n = [ \ 1 \ \exp(\irm\omega_n) \ \cdots \ \exp(\irm(l-1)\omega_n) \ ]^T$. For convenience, let us write the above equation in matrix form. Denoting $\Bx_j = \boldsymbol{\beta}_j\odot\Bh$ as in \eqref{eq2} and $\boldsymbol{\varphi}_m = [ \ \exp(\irm\omega_1m) \ \cdots \ \exp(\irm\omega_{\vert\mathcal{N}\vert}m) \ ]^T$ we can write
\begin{equation}
    \Bs_{m,j} = \boldsymbol{\Theta} \ ( \ \Bx_j\odot\boldsymbol{\varphi}_m \ )
\end{equation}
where $\boldsymbol{\Theta} = [\ \boldsymbol{\theta}_1 \ \cdots \ \boldsymbol{\theta}_{\vert\mathcal{N}\vert} \ ]$ is a Vandermonde matrix. By arranging all snapshots obtained from received signal in $j^{th}$ frame, we can write
\begin{align}
    \bS_j &= [ \ \Bs_{0,j} \ \Bs_{1,j} \ \cdots \ \Bs_{M-l+1,j} \ ]\nonumber\\
    &= \boldsymbol{\Theta} \ [ \ \Bx_j\odot\boldsymbol{\varphi}_0 \ \cdots \ \Bx_j\odot\boldsymbol{\varphi}_{M-l+1} \ ]\nonumber\\
    &= \boldsymbol{\Theta} \ \diag(\Bx_j\odot\boldsymbol{\varphi}_m) \ \boldsymbol{\Gamma}
    \label{model}
\end{align}
In \eqref{model}, both $\boldsymbol{\Theta} \in \mathbb{C}^{ l\times \vert\mathcal{N}\vert}$ and $\boldsymbol{\Gamma} \in \mathbb{C}^{\vert\mathcal{N}\vert \times (M-l+1)}$ are Vandermonde matrix by construction. Finally, gathering all snapshots from all frames \textit{i.e}: $\{ j\}_{j=1}^J$, we obtain the following data matrix $\Tilde{\bS}\in\mathbb{C}^{l \times P}$
\begin{equation}
\Tilde{\bS} = [ \ \bS_1 \ \bS_2 \ \cdots \ \bS_J \ ]
\label{son}
\end{equation}
Hence, the use of sinusoid sequence effectively turns the AUD in UL NOMA problem into a frequency estimation problem. 

==> sections/system_model.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/schematic.pdf}
    \caption{Uplink scenario of an mMTC cell with single BS and $N$ synchronized UEs}
    \label{mMTC}
\end{figure}

Let us consider a cell of an mMTC system consists of single BS, $N$ UEs and $M$ subcarriers where $N>M$ due to scarce resources. This results into non-orthogonal nature of multiple access. The UEs are assumed to be synchronized in time, an approximation shown to have marginal impact on mMTC performance because of small packet sizes (10-100 bytes) \cite{ep}. The number of potential UEs $N$ can be very large but a small fraction of them initiates sporadic transmission at any given point of time \cite{empirical}. This fraction is denoted as activation probability $p_a$. Moreover, we assume flat Rayleigh fading channels in uplink which asserts that all subcarriers fall within coherent bandwidth and channel gains remain unchanged over the all frames. The complex channel coefficients experienced by each of $n$ UE where $\{n\}_{n=1}^N$ are considered to be independent zero mean complex Gaussian random variable \textit{i.e:} $\mathcal{CN}~(h_n\vert 0,\tau)$. The variance $\tau$ captures pathloss exponent considering an NLOS environment and is modeled, as shown in later section, using a pathloss model demonstrated in 3GPP (release 9). 

During random access, an UE transmits over a timeslot consists of $J$ frames. As shown in \ref{mMTC}, first frame includes pilot symbol and following $J-1$ frames carry data symbols. At any time slot $j\in\{ \ 1,2,\cdots \ J \ \}$, the received signal $\By\in\mathbb{C}^M$ at BS can be written as following
\\
\begin{align}
    \By_j &= \sum_{n=1}^{\vert\mathcal{N}\vert} h_n \beta_{n,j} \boldsymbol{\phi}_n + \Bw
    \label{eq1}
\end{align}
\\
where, $\beta_{n,j}$ is data or pilot symbol. In this work we consider QPSK constellation with $\E[\vert\beta_{n,j}\vert^2] = 1$, but it can be generalized for higher order PSK constellations. Moreover, $\mathcal{N}$ denotes the set of active users and $\vert\mathcal{N}\vert$ is the number of active users. $\boldsymbol{\phi}_n \in \mathbb{C}^M$ is the spreading sequence assigned to $n^{th}$ user. Uniform power allocation for all UE is considered, \textit{i.e}: $\{\vert\vert\ \boldsymbol{\phi}_i\vert\vert_2\}_{i=1}^N = \gamma$  In the existing works, Zadoff-Chu or random sequences are the spreading sequence of choice \cite{ulgf_2,ep,sompext}.  Furthermore, $\Bw \sim \mathcal{CN}(\textbf{0},\sigma_w^2\bI_M)$ is receiver noise. \eqref{eq1} can be written as 
\\
\begin{align}
    \By_j = \Phi(\boldsymbol{\beta}_j\odot\Bh) + \Bw\label{eq2}
\end{align}
\\
where $\Phi = [\boldsymbol{\phi}_1, \ \cdots \ ,\boldsymbol{\phi}_{\vert\mathcal{N}\vert}]$, $\boldsymbol{\beta}_j = [ \beta_{1,j}, \ \cdots \ ,\beta_{\vert\mathcal{N}\vert,j}]^T$ and $\Bh = [h_1, \ \cdots \ ,h_{\vert\mathcal{N}\vert}]^T$. \eqref{eq2} can also be written as an undetermined system equations exploiting the fact that $\vert\mathcal{N}\vert \ll N$ to employ CS-MUD techniques \cite{gomp,sompext,ieamp}. Combining all received signals from $\{j\}_{j=1}^J$, we get 
\begin{equation}
    \bY = \Phi\Upsilon + \bW
    \label{father}
\end{equation}
where, $\Upsilon = [\boldsymbol{\beta}_1\odot\Bh \ \cdots \ \boldsymbol{\beta}_J\odot\Bh]$, $\bW\in\mathbb{C}^{M\times J}$ is the combined noise term over all frames. 
